Unified inverse correspondence for LE-logics

We generalize Kracht's theory of internal describability from classical modal logic to the family of all logics canonically associated with varieties of normal lattice expansions (LE algebras). We work in the purely algebraic setting of perfect LEs; the formulas playing the role of Kracht's formulas in this generalized setting pertain to a first order language whose atoms are special inequalities between terms of perfect algebras. Via duality, formulas in this language can be equivalently translated into first order conditions in the frame correspondence languages of several types of relational semantics for LE-logics.

==> sections/instances/graphbased.tex <==
\subsection{Graph based semantics}
\label{ssec:graph_based_semantics}

Graph based semantics were introduced in \cite{conradie2020non} and \mpnote{blablablablabla }

==> sections/instances/polarities_OLD.tex <==
The only difference is that, as opposed for instance to, where $\varphi$  Kripke semantics for modal logic, a sequence of operators of the same type does not correspond to the composition of their associated relations. In particular, the last step of the equivalence chains shown above would be a bit different. For example, a formula such as $\Diamond\Diamond\nomj$ gets interpreted under a valuation $V$ as the concept whose intention is $R_\Diamond^{(0)}[I^{(0)}[R_\Diamond^{(0)}[V(\nomj)]]]$; hence the inequality $\Diamond\Diamond\nomj \leq \cnomm$ is not equivalent to $V(\cnomm) (R_\Diamond \circ R_\Diamond) V(\nomj)$,\footnote{Indeed, $R_\Diamond \circ R_\Diamond$ is usually not even definable as $R_\Diamond \subseteq X\times A$.} but rather to $V(\cnomm) (R_\Diamond ;_I R_\Diamond) V(\nomj)$, where $(R_\Diamond ;_I R_\Diamond)$ denotes the {\em $I$-composition} of $R_\Diamond$ and $R_\Diamond$, i.e., the relation between $X$ and $A$ such that for any $a \in A$, and $x\in X$,\footnote{This type of composition is not new in the literature. It first occurred in \cite{roughconcepts}, and was also studied extensively in \cite{dairapaper}.}
\[
x (R_\Diamond ;_I R_\Diamond) a \quad\quad \mbox{iff} \quad\quad x \in R_\Diamond^{(0)}[I^{(0)}[R_\Diamond^{(0)}[\{a\}]]].
\] 
For simplicity of presentation, we will consider only the case in which the LE signature contains unary operators, but the following discussion can be easily generalized to operators of any arity. Following and extending \cite{dairapaper}, there are six types of $I$-compositions that depend on the type of their operands\footnote{In \cite{roughconcepts} and \cite{dairapaper} the first two of the following $I$-compositions are defined.}. In particular, for any $R_\Diamond \subseteq X \times A$, $R_\lhd \subseteq X \times X$, $R_\Box \subseteq A \times X$, $R_\rhd \subseteq A\times A$, and any $a, b \in A$, $x, y \in X$,
\smallskip

{{\centering
\begin{tabular}{rcl}
$a (R_\Box ;_I R_\Box) x$ & iff & $a \in R_\Box^{(0)}[I^{(1)}[R_\Box^{(0)}[\{x\}]]]$ \\
$x (R_\Diamond ;_I R_\Diamond) a$ & iff & $x \in R_\Diamond^{(0)}[I^{(0)}[R_\Diamond^{(0)}[\{a\}]]]$ \\
$x (R_\lhd ;_I R_\Box) y$ & iff & $a \in R_\lhd^{(0)}[I^{(1)}[R_\Box^{(0)}[\{y\}]]]$ \\
$a (R_\rhd ;_I R_\Diamond) b$ & iff & $x \in R_\rhd^{(0)}[I^{(0)}[R_\Diamond^{(0)}[\{b\}]]]$\\
$x (R_\lhd ;_I R_\rhd) a$ & iff & $x \in R_\lhd^{(0)}[I^{(1)}[R_\rhd^{(0)}[\{a\}]]]$ \\
$a (R_\rhd ;_I R_\lhd) x$ & iff & $a \in R_\rhd^{(0)}[I^{(0)}[R_\lhd^{(0)}[\{x\}]]]$.
\end{tabular}
\par }}
\smallskip

\noindent As discussed above, it is possible to associate a composition of relations to each skeleton formula as follows:

\begin{definition}[Relation associated to a skeleton formula]
\label{def:polarities_rel_associated_to_skeleton}
For any positive definite skeleton formula $\varphi$ and negative definite skeleton formula $\psi$, let $R_\varphi$ and $R_\psi$ be defined as follows by simultaneous recursion.
\begin{description}
    \item[Base case] if $\varphi$ (resp.\ $\psi$) is a variable, $R_\varphi \coloneqq I$ (resp.\ $R_\psi \coloneqq J$);
    \item[Monotone] if $\varphi = \Diamond\varphi'$ (resp.\ $\psi = \Box\psi'$) for some positive (resp.\ negative) skeleton formula $\varphi'$ (resp.\ $\psi'$), then $R_\varphi = R_\Diamond ;_I R_{\varphi'}$ (resp.\ $R_\psi = R_\Box ;_I R_{\psi'})$;
    \item[Antitone] if $\varphi = \lhd\psi'$ (resp.\ $\psi = \rhd\varphi'$) for some negative (resp.\ positive) skeleton formula $\psi'$ (resp.\ $\varphi'$), then $R_\varphi = R_\lhd ;_I R_{\psi'}$ (resp.\ $R_\psi = R_\rhd ;_I R_{\varphi'})$.
\end{description}
\end{definition}


==> sections/inverse/OLD/before_march07.tex <==
\begin{definition}
\label{def:inversedisjunct}
A {\em positive} (resp.\ {\em negative}) {\em inverse disjunct} is a $\langmeta$-formula $\theta^+(\purev)$ (resp.\ $\theta^-(\purev)$) defined inductively together with a pure variable $\purev$. It either is:
\begin{itemize}
    \item an inequality $\purev = \nomj \leq \psi$ or $\varphi \leq \cnomm = \purev$ (resp.\ $\purev = \nomj \nleq \psi$ or $\varphi \nleq \cnomm = \purev$)  such that $\psi$ is a negative skeleton, and $\varphi$ a positive skeleton;
    \item a conjunction (resp.\ disjunction) $\bigmetaand_i \theta_i^+(\purev)$ (resp.\ $\bigmetaor_i \theta_i^-(\purev)$) of inverse disjuncts; 
    \item a quantified formula $\forall\overline\pureu[\nomj \nleq \psi(\overline\pureu) \Rightarrow \bigmetaor_i \theta_i^-(\pureu_i)]$ (resp.\ $\exists \overline\pureu[\bigmetaand_i \theta_i^+(\pureu_i) \metaand \nomj \nleq \psi(\overline\pureu)]$), where $\nomj = \purev$, $\psi$ is a negative skeleton formula, and each $\theta_i^-$ (resp.\ $\theta^+_i$) is a negative (resp.\ positive) inverse disjunct where $\nomj$ does not occur. 
    \item a quantified formula $\forall\overline\pureu[\varphi(\overline\pureu) \nleq \cnomm \Rightarrow \bigmetaor_i \theta_i^-(\pureu_i)]$ (resp.\ $\exists \overline\pureu[\bigmetaand_i \theta_i^+(\pureu_i) \metaand \varphi(\overline\pureu) \nleq \cnomm]$), where $\cnomm = \purev$, $\varphi$ is a positive skeleton formula, and each $\theta_i^-$ (resp.\ $\theta^+_i$) is a negative (resp.\ positive) inverse disjunct where $\cnomm$ does not occur. 
\end{itemize}
\end{definition}

We will always assume that the quantifiers contained in inverse disjuncts introduce fresh variables.

\begin{remark}
\label{remark:restrictedquantifiersnothere}
The cases in Definition \ref{def:inversedisjunct} which contain quantifiers also contain some negated inequality, e.g.\ $\nomj \nleq \psi(\overline\pureu)$ where the negative skeleton contains all (and only) the variables in $\overline\pureu$ that were introduced by the quantifiers of that case. Such inequalities in the classical setting encode relational atoms that {\em restrict} the quantification. For instance, a formula such as $\forall \cnomn(\nomj \nleq \Box \cnomn \Rightarrow \xi)$ in the classical setting would be interpreted as $\forall y(x \nleq \Box y^c \Rightarrow \xi)$ when $\cnomn$ is interpreted as the cosingleton $\{y\}^c$, and $\nomj$ as the singleton $\{x\}$. Hence, it is equivalent to $\forall y(\Box \{y\}^c \leq \{x\}^c \Rightarrow \xi)$, which, as discussed in Remark \ref{remark:flatinequalities}, is equivalent to $\forall y(Rxy \Rightarrow \xi)$, i.e.\ it would be one of Kracht's {\em restricted quantifiers}, namely a quantifier over the successor's of $x$, often denoted as $(\forall y \rhd x)\xi$ \cite{krachtphdthesis,blackburn2002modal}. Kracht's restricted quantifiers have been generalized in \cite{CoPan22} and \cite{inversedle} using inequalities in the language of ALBA. Such inequalities correspond in the classical and distributive case to the {\em restricting inequalities} of Kracht (DLE) disjuncts in \cite{CoPan22,inversedle}. Due to the added complications of the non-distributive setting, and due to the abundance of relational semantics for lattice logics where relational atoms are not expressed uniformly, we have decided not to adopt the terms {\em restricting inequality} and {\em restricted quantifier} in this setting, as they would not represent well the concept of classical restricted quantifier in commonly used semantics for LE-logics. For instance, such inequalities would represent the right type of relational atom in {\em graph based frames}, but their negations in {\em polarity based frames} (see \cite{conradie2020non} for more information on these semantics).
\end{remark}

\begin{lemma}
\label{lemma:compaction}
Every positive (resp.\ negative) inverse disjunct $\theta^+(\purev)$ (resp.\ $\theta^-(\purev)$) is equivalent to some inequality $\nomj \leq \xi$ (resp.\ $\nomj \nleq \xi$) if $\purev$ is some nominal $\nomj$, and to some inequality $\zeta \leq \cnomm$ (resp.\ $\zeta \nleq \cnomm$) if it is some conominal $\cnomm$, where the topmost symbol of $\xi$ is a negative skeleton connective or a pure variable, and the topmost symbol of each $\zeta$ is a positive skeleton connective or a pure variable.
\end{lemma}
\begin{proof}
We proceed by simultaneous induction on the complexity of $\theta^+$ and $\theta^-$ (we do not discuss the cases of $\theta^-$ as they are analogous to those of $\theta^+$). If $\theta^+$ is an inequality $\nomj \leq \varphi$ (resp.\ $\varphi \leq \cnomm)$ such that $\varphi$ is a negative (resp.\ positive) skeleton, we are done, as $\varphi$ is either a pure variable, or its topmost connective is a negative (resp.\ positive) skeleton connective, i.e., a connective in $\mathcal{G}$ or $-\wedge$ (resp.\ $\mathcal{F}$ or $+\vee$). 

If $\theta^+$ is a conjunction of positive inverse disjuncts sharing the same pure variable $\bigmetaand_i^n\theta^+_i(\purev)$, then, by applying the inductive hypothesis on each $\theta^+_i$, it is equivalent to $\bigmetaand_i^n \nomj \leq \xi_i$ (resp.\ $\bigmetaand_i^n \zeta_i \leq \cnomm)$ if $\purev$ is some nominal $\nomj$ (resp.\ conominal $\cnomm$); hence it is equivalent to $\nomj \leq \bigwedge_i^n \xi_i$ (resp.\ $\bigvee_i^n \zeta_i \leq \cnomm$). Since each $\xi_i$ is a finite meet (resp.\ join) of formulas, and its topmost connective is a negative (resp.\ positive) skeleton connective.

Suppose that $\purev$ is some nominal $\nomj$ (resp.\ conominal $\cnomm$) and $\theta^+$ has shape $\forall\overline\pureu(\nomj \nleq \varphi(\overline\pureu) \Rightarrow \bigmetaor^n_i\theta^-_i(\pureu_i))$ (resp.\ $\forall\overline\pureu(\varphi(\overline\pureu) \nleq \cnomm \Rightarrow \bigmetaor^n_i\theta^-_i(\pureu_i))$) such that $\varphi$ is some negative (resp.\ positive) skeleton formula. By taking the contrapositive, $\theta^+$ is equivalent to
\begin{equation}
\label{eq:contrapositive_of_kracht_disjunct}
\forall\overline\pureu(\bigmetaand_i^n\metanot\theta^-_i(\pureu_i) \Rightarrow \nomj \leq \varphi(\overline\pureu)) \quad\quad 
(\mbox{resp.} \ 
\forall\overline\pureu(\bigmetaand_i^n\metanot\theta^-_i(\pureu_i) \Rightarrow \varphi(\overline\pureu) \leq \cnomm),
)
\end{equation}
and by inductive hypothesis, each $\theta_i^-(\pureu_i)$ is equivalent to some inequality $\pureu_i \nleq \xi_i$ if $\pureu_i$ is a nominal, and to some inequality $\zeta_i \nleq \pureu_i$ if it is a conominal; hence $\metanot\theta_i^-(\pureu_i)$ is equivalent to some inequality $\pureu_i \leq \xi_i$ or $\zeta_i \leq \pureu_i$, depending on whether $\pureu_i$ is a nominal or conominal. Let's assume without loss of generality that the first $m$ coordinates of $\varphi$ are positive, and the last $n - m$ are negative. Then \eqref{eq:contrapositive_of_kracht_disjunct} is equivalent to
\[
\forall\overline\pureu(\bigmetaand_{i=1}^m \pureu_i \leq \xi_i
\metaand
\bigmetaand_{i = m+1}^n \zeta_i \leq \pureu_i
\Rightarrow \nomj \leq \varphi(\overline\pureu)) \quad\quad 
(\mbox{resp.} \ 
\forall\overline\pureu(\bigmetaand_{i=1}^m \pureu_i \leq \xi_i
\metaand
\bigmetaand_{i = m+1}^n \zeta_i \leq \pureu_i\Rightarrow \varphi(\overline\pureu) \leq \cnomm),
\]
Then, by Lemma \ref{lemma:firstapprox}, \eqref{eq:contrapositive_of_kracht_disjunct} is equivalent to
$\nomj \leq \varphi(\xi_1,\ldots,\xi_m,\zeta_{m+1},\ldots,\zeta_n)$ (resp.\ $\varphi(\xi_1,\ldots,\xi_m,\zeta_{m+1},\ldots,\zeta_n) \leq \cnomm$), and its topmost connective is a negative (resp.\ positive) skeleton connective.
\end{proof}

==> sections/old/OLD_Things.tex <==
%%%%% OLD LEMMA 50 %%%%%
\begin{lemma}
\label{lemma:compaction}
Every positive (resp.\ negative) inverse disjunct $\theta^+(\purev)$ (resp.\ $\theta^-(\purev)$) is equivalent to some inequality $\nomj \leq \bigwedge_i^n \xi_i$ (resp.\ $\nomj \nleq \bigwedge_i^n \xi_i$) if $\purev$ is some nominal $\nomj$, and to some inequality $\bigvee_i^n \zeta_i \leq \cnomm$ (resp.\ $\bigvee_i^n \zeta_i \nleq \cnomm$) if it is some conominal $\cnomm$, where the topmost symbol of each $\xi_i$ is a connective in $\mathcal{G}$ (resp.\ $\mathcal{F}$) or a pure variable, and the topmost symbol of each $\zeta_i$ is a connective in $\mathcal{F}$ (resp.\ $\mathcal{G}$) or a pure variable.
\end{lemma}
\begin{proof}
We proceed by simultaneous induction on the complexity of $\theta^+$ and $\theta^-$ (we do not discuss the cases of $\theta^-$ as they are analogous to those of $\theta^+$). If $\theta^+$ is an inequality $\nomj \leq \varphi$ (resp.\ $\varphi \leq \cnomm)$ such that $\varphi$ is a negative (resp.\ positive) skeleton, we are done, as $\varphi$ is either a pure variable, or its topmost connective is a negative (resp.\ positive) skeleton connective, i.e., a connective in $\mathcal{G}$ (resp.\ $\mathcal{F}$). 

If $\theta^+$ is a conjunction of positive inverse disjuncts sharing the same pure variable $\bigmetaand_i^n\theta^+_i(\purev)$, then, by applying the inductive hypothesis on each $\theta^+_i$, it is equivalent to $\bigmetaand_i^n \nomj \leq \xi_i$ (resp.\ $\bigmetaand_i^n \zeta_i \leq \cnomm)$ if $\purev$ is some nominal $\nomj$ (resp.\ conominal $\cnomm$); hence it is equivalent to $\nomj \leq \bigwedge_i^n \xi_i$ (resp.\ $\bigvee_i^n \zeta_i \leq \cnomm$). Since each $\xi_i$ is a finite meet (resp.\ join) of formulas whose topmost symbol is a connective in $\mathcal{G}$ (resp.\ $\mathcal{F}$) or a pure variable, the same property holds also for $\bigwedge_i^n\xi_i$ (resp.\ $\bigvee_i^n \zeta_i$).

Suppose that $\purev$ is some nominal $\nomj$ (resp.\ conominal $\cnomm$) and $\theta^+$ has shape $\forall\overline\pureu(\nomj \nleq \varphi(\overline\pureu) \Rightarrow \bigmetaor^n_i\theta^-_i(\pureu_i))$ (resp.\ $\forall\overline\pureu(\varphi(\overline\pureu) \nleq \cnomm \Rightarrow \bigmetaor^n_i\theta^-_i(\pureu_i))$) such that $\varphi$ is some negative (resp.\ positive) skeleton formula. By taking the contrapositive, $\theta^+$ is equivalent to
\begin{equation}
\label{eq:contrapositive_of_kracht_disjunct}
\forall\overline\pureu(\bigmetaand_i^n\metanot\theta^-_i(\pureu_i) \Rightarrow \nomj \leq \varphi(\overline\pureu)) \quad\quad 
(\mbox{resp.} \ 
\forall\overline\pureu(\bigmetaand_i^n\metanot\theta^-_i(\pureu_i) \Rightarrow \varphi(\overline\pureu) \leq \cnomm),
)
\end{equation}
and by inductive hypothesis, each $\theta_i^-(\pureu_i)$ is equivalent to some inequality $\pureu_i \nleq \xi_i$ if $\pureu_i$ is a nominal, and to some inequality $\zeta_i \nleq \pureu_i$ if it is a conominal; hence $\metanot\theta_i^-(\pureu_i)$ is equivalent to some inequality $\pureu_i \leq \xi_i$ or $\zeta_i \leq \pureu_i$, depending on whether $\pureu_i$ is a nominal or conominal. Let's assume without loss of generality that the first $m$ coordinates of $\varphi$ are positive, and the last $n - m$ are negative. Then \eqref{eq:contrapositive_of_kracht_disjunct} is equivalent to
\[
\forall\overline\pureu(\bigmetaand_{i=1}^m \pureu_i \leq \xi_i
\metaand
\bigmetaand_{i = m+1}^n \zeta_i \leq \pureu_i
\Rightarrow \nomj \leq \varphi(\overline\pureu)) \quad\quad 
(\mbox{resp.} \ 
\forall\overline\pureu(\bigmetaand_{i=1}^m \pureu_i \leq \xi_i
\metaand
\bigmetaand_{i = m+1}^n \zeta_i \leq \pureu_i\Rightarrow \varphi(\overline\pureu) \leq \cnomm),
\]
Then, by Corollary \ref{cor:firstapprox_inductive}, \eqref{eq:contrapositive_of_kracht_disjunct} is equivalent to
$\nomj \leq \varphi(\xi_1,\ldots,\xi_m,\zeta_{m+1},\ldots,\zeta_n)$ (resp.\ $\varphi(\xi_1,\ldots,\xi_m,\zeta_{m+1},\ldots,\zeta_n) \leq \cnomm$), and its topmost connective is in $\mathcal{G}$ (resp.\ $\mathcal{F}$) since $\varphi$ is a negative (resp.\ positive) skeleton formula.
\end{proof}

==> sections/old/old_fisher_servi.tex <==
We analyze the Fisher Servi inequality both in the distributive setting of intuitionistic modal logic where $\mathcal{F} = \{\Diamond, \wedge\}$ and $\mathcal{G} = \{\Box, \rightarrow, \vee\}$, and a non-distributive one where $\mathcal{F} = \{\Diamond\}$ and $\mathcal{G} = \{\Box, \backslash \}$.

\paragraph{Inequalities.} Distributive setting: $\Diamond(p \rightarrow q) \leq \Box p \rightarrow \Diamond q$ with $\varepsilon(p,q) = (1,1)$ and $p <_\Omega q$, \\
Non-distributive setting: $\Diamond(p \backslash q) \leq \Box p \backslash \Diamond q$ with $\varepsilon(p,q) = (1,1)$ and $p <_\Omega q$.

\paragraph{ALBA Runs.} Distributive:
\smallskip

{{\centering
\begin{tabular}{rl}
& $\Diamond(p \rightarrow q) \leq \Box p \rightarrow \Diamond q$ \\
& $\forall \nomj_1, \nomj_2, \cnomm_1(\nomj_1 \leq p \rightarrow q \metaand \nomj_2 \leq \Box p \metaand \Diamond q \leq \cnomm_1 \Rightarrow \Diamond\nomj_1 \leq \nomj_2 \rightarrow \cnomm_1)$ \\
& $\forall \nomj_1, \nomj_2, \cnomm_1(\nomj_1 \wedge p \leq q \metaand \Diamondblack\nomj_2 \leq p \metaand \Diamond q \leq \cnomm_1 \Rightarrow \Diamond\nomj_1 \leq \nomj_2 \rightarrow \cnomm_1)$ \\
& $\forall \nomj_1, \nomj_2, \cnomm_1( \Diamond (\nomj_1 \wedge \Diamondblack\nomj_2) \leq \cnomm_1 \Rightarrow \Diamond\nomj_1 \leq \nomj_2 \rightarrow \cnomm_1)$
\end{tabular}
\par}}
\smallskip

\noindent Non-Distributive:
\smallskip

{{\centering
\begin{tabular}{rl}
& $\Diamond(p \backslash q) \leq \Box p \backslash \Diamond q$ \\
& $\forall \nomj_1, \nomj_2, \cnomm_1(\nomj_1 \leq p \backslash q \metaand \nomj_2 \leq \Box p \metaand \Diamond q \leq \cnomm_1 \Rightarrow \nomj_1 \leq \nomj_2 \backslash \cnomm_1)$ \\
& $\forall \nomj_1, \nomj_2, \cnomm_1(\nomj_1 \circ p \leq q \metaand \Diamondblack\nomj_2 \leq p \metaand \Diamond q \leq \cnomm_1 \Rightarrow \nomj_1 \leq \nomj_2 \backslash \cnomm_1)$ \\
& $\forall \nomj_1, \nomj_2, \cnomm_1( \Diamond (\nomj_1 \circ \Diamondblack\nomj_2) \leq \cnomm_1 \Rightarrow \nomj_1 \leq \nomj_2 \backslash \cnomm_1)$
\end{tabular}
\par}}
\smallskip

\paragraph{Flattifications.} Distributive: already flat according to the definitions in this paper. Using the procedures in \cite{inversedle}, we could further flattify as follows 
\smallskip

{{\centering
\begin{tabular}{rl}
& $\forall \nomj_1, \nomj_2, \cnomm_1( \Diamond (\nomj_1 \wedge \Diamondblack\nomj_2) \leq \cnomm_1 \Rightarrow \Diamond\nomj_1 \leq \nomj_2 \rightarrow \cnomm_1)$ \\
& $\forall \nomj_1, \nomj_2, \cnomm_1( \Diamond (\Diamond\nomj_1 \nleq \nomj_2 \rightarrow \cnomm_1 \Rightarrow \nomj_1 \wedge \Diamondblack\nomj_2) \nleq \cnomm_1 )$ \\
& $\forall \nomj_1, \nomj_2, \nomj_3, \cnomm_1( \nomj_3 \leq \Diamond\nomj_1 \metaand \nomj_3 \nleq \nomj_2 \rightarrow \cnomm_1 \Rightarrow \Diamond(\nomj_1 \wedge \Diamondblack\nomj_2) \nleq \cnomm_1 )$ \\
& $\forall \nomj_1, \nomj_2, \nomj_3, \cnomm_1( \nomj_3 \leq \Diamond\nomj_1  \metaand \nomj_2 \rightarrow \cnomm_1 \leq \kappa \nomj_3 \Rightarrow \lambda\cnomm_1 \leq \Diamond(\nomj_1 \wedge \Diamondblack\nomj_2))$ \\
& $\forall \nomj_1, \nomj_2, \nomj_3, \cnomm_1( \nomj_3 \leq \Diamond\nomj_1  \metaand \nomj_2 \rightarrow \cnomm_1 \leq \kappa \nomj_3 \Rightarrow  (\exists \nomi \rhd_\Diamond \lambda\cnomm_1) \nomi \leq \nomj_1 \wedge \Diamondblack\nomj_2))$  \\
& $\forall \nomj_1, \nomj_2, \nomj_3 \cnomm_1( \nomj_3 \leq \Diamond\nomj_1  \metaand \nomj_2 \rightarrow \cnomm_1 \leq \kappa \nomj_3 \Rightarrow (\exists \nomi \rhd_\Diamond \lambda\cnomm_1)(\nomi \leq \nomj_1 \metaand \nomi \leq \Diamondblack\nomj_2))$,
\end{tabular}
\par}}
\smallskip

\noindent where $\kappa$ and $\lambda$ are two isomorphisms between completely join and meet irreducibles, and $(\exists \nomi \rhd_\Diamond \lambda \cnomm_1)\varphi := \exists \nomi(\nomi \leq \Diamond \lambda\cnomm_1 \wedge \varphi)$.

Non distributive: already flat.

\paragraph{Inverse correspondence.} Distributive:
\smallskip

{{\centering 
\begin{tabular}{rl}
& $\forall \nomj_1, \nomj_2, \cnomm_1( \Diamond (\nomj_1 \wedge \Diamondblack\nomj_2) \leq \cnomm_1 \Rightarrow \Diamond\nomj_1 \leq \nomj_2 \rightarrow \cnomm_1)$ \\
iff & $\forall \nomj_1, \nomj_2, \cnomm_1( \Diamond (p_{\nomj_1} \wedge \Diamondblack p_{\nomj_2}) \leq \cnomm_1 \metaand \nomj_1 \leq p_{\nomj_1} \metaand \nomj_2 \leq p_{\nomj_2} \Rightarrow \Diamond\nomj_1 \leq \nomj_2 \rightarrow \cnomm_1)$ \\
iff & $\Diamond p_{\nomj_1} \leq p_{\nomj_2} \rightarrow \Diamond (p_{\nomj_1} \wedge \Diamondblack p_{\nomj_2})$
\end{tabular}
\par}}
\smallskip

\noindent Non Distributive:
\smallskip

{{\centering 
\begin{tabular}{rl}
& $\forall \nomj_1, \nomj_2, \cnomm_1( \Diamond (\nomj_1 \circ \Diamondblack\nomj_2) \leq \cnomm_1 \Rightarrow \Diamond\nomj_1 \leq \nomj_2 \backslash \cnomm_1)$ \\
iff & $\forall \nomj_1, \nomj_2, \cnomm_1( \Diamond (p_{\nomj_1} \circ \Diamondblack p_{\nomj_2}) \leq \cnomm_1 \metaand \nomj_1 \leq p_{\nomj_1} \metaand \nomj_2 \leq p_{\nomj_2} \Rightarrow \Diamond\nomj_1 \leq \nomj_2 \backslash \cnomm_1)$ \\
iff & $\Diamond p_{\nomj_1} \leq p_{\nomj_2} \backslash \Diamond (p_{\nomj_1} \circ \Diamondblack p_{\nomj_2})$
\end{tabular}
\par}}
\smallskip

\noindent

\paragraph{Crypto step.} The inequality is crypto inductive for $\varepsilon(p_{\nomj_1},p_{\nomj_2}) = (1, 1)$ and $p_{\nomj_1} <_\Omega p_{\nomj_2}$.

Distributive:
\smallskip

{{\centering 
\begin{tabular}{rl}
& $\Diamond p_{\nomj_1} \leq p_{\nomj_2} \rightarrow \Diamond (p_{\nomj_1} \wedge \Diamondblack p_{\nomj_2})$ \\
iff & $p_{\nomj_1} \leq v_1 \metaand \Diamondblack p_{\nomj_2} \leq v_2 \metaand  \Rightarrow \Diamond p_{\nomj_1} \leq p_{\nomj_2} \rightarrow \Diamond (v_1 \wedge v_2)$ \\ 
iff & $p_{\nomj_1} \leq v_1 \metaand p_{\nomj_2} \leq \Box v_2 \metaand  \Rightarrow \Diamond p_{\nomj_1} \leq p_{\nomj_2} \rightarrow \Diamond (v_1 \wedge v_2)$ \\
iff & $\Diamond v_1 \leq \Box v_2 \rightarrow \Diamond (v_1 \wedge v_2)$,
\end{tabular}
\par}}
\smallskip

\noindent i.e., one of Dunn's axioms for positive modal logic.

\noindent Non Distributive:
\smallskip

{{\centering 
\begin{tabular}{rl}
& $\Diamond p_{\nomj_1} \leq p_{\nomj_2} \backslash \Diamond (p_{\nomj_1} \circ \Diamondblack p_{\nomj_2})$ \\
iff & $p_{\nomj_1} \leq v_1 \metaand v_1 \circ \Diamondblack p_{\nomj_2} \leq v_2 \metaand  \Rightarrow \Diamond p_{\nomj_1} \leq p_{\nomj_2} \backslash \Diamond v_2$ \\ 
iff & $p_{\nomj_1} \leq v_1 \metaand p_{\nomj_2} \leq \Box (v_1 \backslash v_2) \metaand  \Rightarrow \Diamond p_{\nomj_1} \leq p_{\nomj_2} \backslash \Diamond v_2$ \\
iff & $p_{\nomj_2} \leq \Box (v_1 \backslash v_2) \metaand  \Rightarrow \Diamond v_1 \leq p_{\nomj_2} \backslash \Diamond v_2$ \\
iff & $\Diamond v_1 \leq \Box (v_1 \backslash v_2) \backslash \Diamond v_2$
\end{tabular}
\par}}
\smallskip

\paragraph{Instantiation to Kripke.} We consider the flattified version of the distributive setting:
\[
\forall \nomj_1, \nomj_2, \nomj_3, \cnomm_1( \nomj_3 \leq \Diamond\nomj_1  \metaand \nomj_2 \rightarrow \cnomm_1 \leq \kappa \nomj_3 \Rightarrow \lambda\cnomm_1 \leq (\exists \nomi \rhd_\Diamond \lambda\cnomm_1)(\nomi \leq \nomj_1 \metaand \nomi \leq \Diamondblack\nomj_2)).
\]
Let us associate a world to each nominal and conominal, e.g., $\nomj_1 \mapsto x$, $\nomj_2 \mapsto y$, $\nomj_3 \mapsto z$, $\cnomm \mapsto w^c$. Then, it becomes
\[
\forall x,y,z,w( z R_\Diamond x  \metaand y=w=z \Rightarrow (\exists v \rhd_\Diamond w)(v = x \metaand y R_\Box x)),
\]
which can be simplified to
\[
\forall x,y( y R_\Diamond x  \Rightarrow  y R_\Box x).
\]

\paragraph{Instantiation to Polarities.}
We consider the flattified version of the non-distributive setting and proceed as outlined in Section \ref{ssec:polarity_based_semantics}:
\smallskip

{{\centering
\begin{tabular}{rl}
& $\forall \nomj_1, \nomj_2, \cnomm_1( \Diamond (\nomj_1 \circ \Diamondblack\nomj_2) \leq \cnomm_1 \Rightarrow \Diamond\nomj_1 \leq \nomj_2 \backslash \cnomm_1)$ \\
iff & $\forall \nomj_1, \nomj_2, \cnomm_1,\cnomm_2( \Diamond (\nomj_1 \circ \Diamondblack\nomj_2) \leq \cnomm_1 \metaand \nomj_2 \backslash \cnomm_1 \leq \cnomm_2 \Rightarrow \Diamond\nomj_1 \leq \cnomm_2)$ \\
i.e. & $\forall a, b, x, y (R_{\Diamond (\cdot \circ \Diamondblack\cdot)}(x, a, b) \metaand R_\backslash(y, b, x) \Rightarrow R_\Diamond(a, y))$ \\
iff & $\forall a, b, x, y (
x \in R_\Diamond^{(0)}[R_{(\cdot \circ \Diamondblack\cdot)}^{(0)}[a, b]^\downarrow]
\metaand R_\backslash(y, b, x) \Rightarrow R_\Diamond(a, y))$ \\
iff & $\forall a, b, x, y (
x \in R_\Diamond^{(0)}[R_{\circ}^{(0)}[a, R_{\Diamondblack}^{(0)}[b]^\downarrow]^\downarrow]
\metaand R_\backslash(y, b, x) \Rightarrow R_\Diamond(a, y))$\\
iff & $\forall a, b, x, y (
\forall c(c \in R_{\circ}^{(0)}[a, R_{\Diamondblack}^{(0)}[b]^\downarrow]^\downarrow \Rightarrow xR_\Diamond c)
\metaand R_\backslash(y, b, x) \Rightarrow R_\Diamond(a, y))$.\\
\end{tabular}
\par}}
